Memory Networks

We describe a new class of learning models called memory networks. Memory networks reason with inference components combined with a long-term memory component; they learn how to use these jointly. The long-term memory can be read and written to, with the goal of using it for prediction. We investigate these models in the context of question answering (QA) where the long-term memory effectively acts as a (dynamic) knowledge base, and the output is a textual response. We evaluate them on a large-scale QA task, and a smaller, but more complex, toy task generated from a simulated world. In the latter, we show the reasoning power of such models by chaining multiple supporting sentences to answer questions that require understanding the intension of verbs.

==> macro.tex <==
% datasets
\newcommand{\fb}{{\sc Freebase}\xspace}
\newcommand{\dbp}{{\sc DBPedia}\xspace}
\newcommand{\wk}{{\sc WikiAnswers}\xspace}
\newcommand{\wq}{{\sc WebQuestions}\xspace}
\newcommand{\rv}{{\sc ReVerb}\xspace}
\newcommand{\cw}{{\sc ClueWeb}\xspace}



% methods
\newcommand{\us}{Our approach}

% commands
\newcommand{\ent}[1]{{\small {\tt #1}}}
